TwinRAN: Twinning the 5G RAN in Azure Cloud

The proliferation of 5G technology necessitates advanced network management strategies to ensure optimal performance and reliability. Digital Twin (DT)s have emerged as a promising paradigm for modeling and simulating complex systems like the 5G Radio Access Network (RAN). In this paper, we present TwinRAN, a DT of the 5G RAN built leveraging the Azure DT platform. TwinRAN is built on top of the Open RAN (O-RAN) architecture and is agnostic to the vendor of the underlying equipment. We demonstrate three applications using TwinRAN and evaluate the required resources and their performance for a network with 800 users and eight gNBs. We first evaluate the performance and limitations of the Azure DT platform, measuring the latency under different conditions. The results from this evaluation allow us to optimize TwinRAN for the DT platform it uses. Then, we present the system's architectural design, emphasizing its components and interactions. We propose that two types of twin graphs be simultaneously maintained on the cloud: one for intercell operations, keeping a broad overview of all the cells in the network, and another where each cell is spawned in a separate Azure DT instance for more granular operation and monitoring of intracell tasks. We evaluate the performance and operating costs of TwinRAN for each of the three applications. The TwinRAN DT in the cloud can keep track of its physical twin within a few hundred milliseconds, extending its utility to many 5G network management tasks, some of which are shown in this paper. The novel framework for building and maintaining a DT of the 5G RAN presented in this paper offers network operators enhanced capabilities, empowering efficient deployments and management.

==> Tables/big_models.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|ccc||ccc}
\hline
\multicolumn{3}{|c|}{\textbf{gNB}}                                                                                                                     & \multicolumn{3}{c|}{\textbf{UE}}                                                                                    \\ \hline
\multicolumn{1}{|c|}{\textbf{Property}} & \multicolumn{1}{c|}{\textbf{Schema}} & \textbf{\begin{tabular}[c]{@{}c@{}}Range or\\ Candidate\end{tabular}} & \multicolumn{1}{c|}{\textbf{Property}} & \multicolumn{1}{c|}{\textbf{Schema}} & \multicolumn{1}{c|}{\textbf{Range}} \\ \hline
\multicolumn{1}{|c|}{Tx Power}          & \multicolumn{1}{c|}{float}           & 20-50                                                                 & \multicolumn{1}{c|}{RNTI}              & \multicolumn{1}{c|}{int}             & \multicolumn{1}{c|}{0-999}          \\ \hline
\multicolumn{1}{|c|}{Connected UEs}     & \multicolumn{1}{c|}{int}             & 0-99                                                                  & \multicolumn{1}{c|}{Location}          & \multicolumn{1}{c|}{Geospatial}      & \multicolumn{1}{c|}{-}              \\ \hline
\multicolumn{1}{|c|}{Relationship}      & \multicolumn{1}{c|}{float}           & gNB                                                                   & \multicolumn{1}{c|}{RSRP}              & \multicolumn{1}{c|}{int}             & \multicolumn{1}{c|}{30.0 - 160.0}   \\ \hline
\multicolumn{1}{|c|}{UE1}               & \multicolumn{1}{c|}{Component}       & UE                                                                    &                                        &                                      &                                     \\ \cline{1-3}
\multicolumn{1}{|c|}{UE2}               & \multicolumn{1}{c|}{Component}       & UE                                                                    &                                        &                                      &                                     \\ \cline{1-3}
\multicolumn{1}{|c|}{...}               & \multicolumn{1}{c|}{...}             & ...                                                                   &                                        &                                      &                                     \\ \cline{1-3}
\multicolumn{1}{|c|}{UE 99}             & \multicolumn{1}{c|}{Component}       & UE                                                                    &                                        &                                      &                                     \\ \cline{1-3}
\end{tabular}
}
\caption{\small{DTDL Interfaces for the TwinRAN-multi instance. The UE is contained in the gNB using the DTDL \textit{component} metaclass. Thus, all the parameters here are contained in a single twin.}}
\label{tab:big_model}
\end{table}

==> Tables/gnbmodels.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Attribute} & \textbf{O-RAN Message} \\ \hline
Cell ID            & E2 Setup Request       \\ \hline
PLMN MCC           & E2 Setup Request       \\ \hline
PLMN MNC           & E2 Setup Request       \\ \hline
Num UEs            & Indication Message     \\ \hline
\end{tabular}
\caption{Minimum DTDL Model of the gNB in TwinRAN. All the attributes are of Integer datatype. In DTDL, one can also limit values within a certain range. The Azure DT instance checks the datatype and range before updating the DT in the live execution environment. }
\label{tab:gnbmodel}
\end{table}

==> Tables/small_models.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccc||ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{gNB}}                                                                                                                     & \multicolumn{3}{c|}{\textbf{UE}}                                                               \\ \hline
\multicolumn{1}{|c|}{\textbf{Property}} & \multicolumn{1}{c|}{\textbf{Schema}} & \textbf{\begin{tabular}[c]{@{}c@{}}Range or\\ Candidate\end{tabular}} & \multicolumn{1}{c|}{\textbf{Property}} & \multicolumn{1}{c|}{\textbf{Schema}} & \textbf{Range} \\ \hline
\multicolumn{1}{|c|}{PLMN}              & \multicolumn{1}{c|}{int}             & 20-50                                                                 & \multicolumn{1}{c|}{RNTI}              & \multicolumn{1}{c|}{int}             & 0-999          \\ \hline
\multicolumn{1}{|c|}{Connected UEs}     & \multicolumn{1}{c|}{int}             & 0-99                                                                  & \multicolumn{1}{c|}{Location}          & \multicolumn{1}{c|}{Geospatial}      & -              \\ \hline
\multicolumn{1}{|c|}{Relationship}      & \multicolumn{1}{c|}{bool}             & UE                                                                    & \multicolumn{1}{c|}{Buffer}            & \multicolumn{1}{c|}{int}             & 0-255          \\ \hline
\multicolumn{1}{|c|}{ARFCN}             & \multicolumn{1}{c|}{int}             & 600000 – 2016666                                                      & \multicolumn{1}{c|}{UL BLER}           & \multicolumn{1}{c|}{float}           & 0.0-1.0        \\ \hline
                                        &                                      &                                                                       & \multicolumn{1}{c|}{UL CQI}            & \multicolumn{1}{c|}{int}             & 0-15           \\ \cline{4-6} 
                                        &                                      &                                                                       & \multicolumn{1}{c|}{DL BLER}           & \multicolumn{1}{c|}{float}           & 0.0-1.0        \\ \cline{4-6} 
                                        &                                      &                                                                       & \multicolumn{1}{c|}{DL MCS}            & \multicolumn{1}{c|}{int}             & 0-15           \\ \cline{4-6} 
\end{tabular}
}
\caption{\small{DTDL Interfaces for the TwinRAN-cell instances. Every instance has one gNB and $N \leq 99$ UEs. The \textit{relationship} defines whether the UE is connected to the gNB.}}
\label{tab:small_models}
\end{table}

==> Tables/uemodels.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Attribute} & \textbf{Datatype} & \textbf{Range} \\ \hline
RNTI               & int               & 0-9999          \\ \hline
DL BLER            & float             & 0.00-1.00      \\ \hline
UL BLER            & float             & 0.00-1.00      \\ \hline
DL MCS             & int               & 1-28           \\ \hline
UL MCS             & int               & 1-28           \\ \hline
DL CQI             & int               & 0-15           \\ \hline
UL CQI             & int               & 0-15           \\ \hline
Buffer Size        & int               & 0-255          \\ \hline

\end{tabular}
\caption{Minimum DTDL Model of the UE in TwinRAN. The datatypes and ranges defined in DTDL help maintain a consistent Azure cloud model. In DTDL the dataypes are called \textit{schema}. }
\label{tab:uemodel}
\end{table}
